Enhancing Multi-Class Anomaly Detection via Diffusion Refinement with Dual Conditioning

Anomaly detection, the technique of identifying abnormal samples using only normal samples, has attracted widespread interest in industry. Existing one-model-per-category methods often struggle with limited generalization capabilities due to their focus on a single category, and can fail when encountering variations in product. Recent feature reconstruction methods, as representatives in one-model-all-categories schemes, face challenges including reconstructing anomalous samples and blurry reconstructions. In this paper, we creatively combine a diffusion model and a transformer for multi-class anomaly detection. This approach leverages diffusion to obtain high-frequency information for refinement, greatly alleviating the blurry reconstruction problem while maintaining the sampling efficiency of the reverse diffusion process. The task is transformed into image inpainting to disconnect the input-output correlation, thereby mitigating the "identical shortcuts" problem and avoiding the model from reconstructing anomalous samples. Besides, we introduce category-awareness using dual conditioning to ensure the accuracy of prediction and reconstruction in the reverse diffusion process, preventing excessive deviation from the target category, thus effectively enabling multi-class anomaly detection. Futhermore, Spatio-temporal fusion is also employed to fuse heatmaps predicted at different timesteps and scales, enhancing the performance of multi-class anomaly detection. Extensive experiments on benchmark datasets demonstrate the superior performance and exceptional multi-class anomaly detection capabilities of our proposed method compared to others.

==> exp/exp_det_btad.tex <==

\begin{table}[t]
	\centering
	\small
	\caption{\textbf{Anomaly detection results with AUROC metric on BTAD} under the unified case.}
	\resizebox{0.5\textwidth}{!}{
		\begin{tabular}{cc|ccc|c}
			\toprule
			Metric & Method & 1 & 2 & 3 & Avg \\
			\midrule
			\multirow{6}{*}{\shortstack{Image-wise\\AUROC}} & UniAD~\cite{uniad} & 99.51 & 76.96 & 98.83 & 91.77 \\
			&UniAD(56$\times$56) & 99.12 & 78.10 & 98.84 & 92.02 \\
			&UniAD+VAE & 99.77 & 77.33 & 99.81 & 92.30 \\
			&UniAD+GAN & 98.15 & 77.95 &  \textbf{99.82} & 91.97 \\
			&UniAD+UNet & 97.95 & 78.78 & 98.97 & 91.90 \\
			% \cmidrule(lr){2-6}
			&Ours & \textbf{99.81} & \textbf{82.07} & {98.88} & \textbf{93.59} \\
			\midrule
			\multirow{6}{*}{\shortstack{Pixel-wise\\AUROC}} & UniAD~\cite{uniad} & 97.00 & 95.14 & 98.63 & 96.92 \\
			&UniAD(56$\times$56) & 97.55 & 95.06 & 98.70 & 97.10 \\
			&UniAD+VAE & 96.92 & 94.90 & \textbf{99.68} & 97.17 \\
			&UniAD+GAN & 96.95  & 94.69 & 99.57 & 97.07 \\
			&UniAD+UNet & 97.02 & 94.81 & 99.46 & 97.13 \\
			% \cmidrule(lr){2-6}
			&Ours & \textbf{98.53} & \textbf{96.75} & 99.50 & \textbf{98.26} \\
			\bottomrule
		\end{tabular}
	}
 	\label{tab:btad}

\end{table}


==> exp/exp_det_loc_mvtec.tex <==

\begin{table*}[t]
	\setlength\tabcolsep{2.0pt}
	\centering
	% \small
	\scriptsize
	\caption{\textbf{Anomaly detection results (det) and localization results (loc) with AUROC metric on MVTec-AD}. All methods are evaluated under the unified case, where the learned model is applied to detect anomalies for all categories \textit{without} fine-tuning.}
	\resizebox{\textwidth}{!}{
		\begin{tabular}{c||cc|cc|cc|cc|cc|cc|cc|cc|cc|cc||cc|cc|cc|cc|cc||cc}
			\toprule
			% \multicolumn{2}{c|}{Category} & US & PSVDD & PaDiM & CutPaste & MKD & DR$\AE$M & UniAD & Ours \\
			\multirow{3}{*}{Method} & \multicolumn{20}{c||}{Object} & \multicolumn{10}{c||}{Texture} &  &\\
			% \Xcline{2-16}{0.5pt}
			& \multicolumn{2}{c|}{Bottle} & \multicolumn{2}{c|}{Cable} & \multicolumn{2}{c|}{Capsule} & \multicolumn{2}{c|}{Hazelnut} & \multicolumn{2}{c|}{MetalNut} & \multicolumn{2}{c|}{Pill} & \multicolumn{2}{c|}{Screw} & \multicolumn{2}{c|}{Toothbrush} & \multicolumn{2}{c|}{Transistor} & \multicolumn{2}{c||}{Zipper} & \multicolumn{2}{c|}{Carpet} & \multicolumn{2}{c|}{Grid} & \multicolumn{2}{c|}{Leather} & \multicolumn{2}{c|}{Tile} & \multicolumn{2}{c||}{Wood} & \multicolumn{2}{c}{Avg}   \\ 
			&det&loc&det&loc&det&loc&det&loc&det&loc&det	&loc&det&loc&det&loc&det&loc&det&loc&det&loc&det&loc&det&loc&det&loc&det&loc&det&loc \\
			\midrule
			Student-Teacher & 84	&67.9	&60	&78.3	&57.6	&85.5	&95.8	&93.7	&62.7	&76.6	&56.1	&80.3	&66.9	&90.8	&57.8	&86.9	&61	&68.3	&78.6	&84.2	&86.6	&88.7	&69.2	&64.5	&97.2	&95.4	&93.7	&82.7	&90.6	&83.3	&74.5	&81.8  \\
			PatchSVDD &85.5	&86.7	&64.4	&62.2	&61.3	&83.1	&83.9	&97.4	&80.9	&96	&89.4	&96.5	&80.9	&74.3	&99.4	&98	&77.5	&78.5	&77.8	&95.1	&63.3	&78.6	&66	&70.8	&60.8	&93.5	&88.3	&92.1	&72.1	&80.7	&76.8	&85.6  \\ 
			PaDiM & 97.9	&96.1	&70.9	&81	&73.4	&96.9	&85.5	&96.3	&88	&84.8	&68.8	&87.7	&56.9	&94.1	&95.3	&95.6	&86.6	&92.3	&79.7	&94.8	&93.8	&97.6	&73.9	&71	&99.9	&84.8	&93.3	&80.5	&98.4	&89.1	&84.2	&89.5  \\ 
			%CutPaste & 67.9	& -	& 69.2	& -	& 63	& -	& 80.9	& -	& 60	& -	& 71.4	& -	& 85.2	& -	& 63.9	& -	& 57.9	& -	& 93.5	& -	& 93.6	& -	& 93.2	& -	& 93.4	& -	& 88.6	& -	& 80.4	& -	& 77.5	& -  \\ 
			%FCDD &-	&56	&-	&64.1	&-	&67.6	&-	&79.3	&-	&57.5	&-	&65.9	&-	&67.2	&-	&60.8	&-	&54.2	&-	&63	&-	&68.6	&-	&65.8	&-	&66.3	&-	&59.3	&-	&53.3	&-	&63.3 \\
			MKD & 98.7	&91.8	&78.2	&89.3	&68.3	&88.3	&97.1	&91.2	&64.9	&64.2	&79.7	&69.7	&75.6	&92.1	&75.3	&88.9	&73.4	&71.7	&87.4	&86.1	&69.8	&95.5	&83.8	&82.3	&93.6	&96.7	&89.5	&85.3	&93.4	&80.5	&81.9	&84.9  \\ 
			DR{\AE}M & 97.5	&87.6	&57.8	&71.3	&65.3	&50.5	&93.7	&96.9	&72.8	&62.2	&82.2	&94.4	&92	&95.5	&90.6	&97.7	&74.8	&64.5	&98.8	 &{98.3} 	&98	 &{98.6} 	 &{99.3} 	& \textbf{98.7} 	&98.7	&97.3	 &{99.8} 	 &\textbf{98.0} 	 &\textbf{99.8} 	 &\textbf{96.0} 	&88.1	&87.2  \\ 
			AST &96.9	&76.3	&92.3	&91.3	&93.6	&92.6	&98.6	&92.2	&98.8	&87.7	&84.9	&67.4	&92	&82.5	&97.2	&95.5	&96.1	&93	&86.2	&79.5	&97.6	&94.8	&93.4	&85.7	&99.4	&88.6	&96.6	&88.1	&98.2	&77	&94.7	&86.1 \\
			SimpleNet & 97.6	&94.3	&90.9	&91.3	&67.2	&95.3	&99	&95	&97.2	&91	&71.7	&88.9	&50.2	&93	&90	&95.2	&93.6	&91	&98.4	&96.3	&95.7	&97.6	&58.3	&49.5	&97.1	&97.1	&99.2	&93.6	&99.4	&88.8	&87	&90.5 \\
			\midrule
			UniAD & 99.7	&98.1	&95.2	 &\textbf{97.3} 	&86.9	&98.5	&99.8	&98.1	&99.2	&94.8	&93.7	&95	&87.5	&98.3	&94.2	&98.4	&99.8	&97.9	&95.8	&96.8	&99.8	&98.5	&98.2	&96.5	 &\textbf{100} 	&98.8	&99.3	&91.8	&98.6	&93.2	&96.5	&96.8  \\ 
			UniAD(28$\times$28) &99.8	&97.9	 &\textbf{96.4} 	&97	&83.2	&98.2	&99.9	&98.4	&98.2	&94.4	&82.1	&90.7	&90.6	&98.7	&93.3	&98.5	&99.8	&96.1	&94.1	&96.7	 &{99.9} 	&98.5	&93.6	&86.5	 &\textbf{100} 	&99.1	&99.1	&89.3	&98.2	&93.5	&95.2	&95.6  \\ 
			UniAD(56$\times$56) &99.5	&97.6	&95.7	&96.6	&82.3	&97.9	&99.8	&98.5	&98.4	&94	&67.5	&90	&86.7	&98.1	&93.3	&98.2	&99.8	&96.8	&92.3	&96.1	 &\textbf{100} 	 &\textbf{98.7}  	&\textbf{99.7} 	&94.7	 &\textbf{100} 	& \textbf{99.2} 	&98	&88.9	&97.9	&93.5	&94.1	&95.9  \\ 
			UniAD+VAE &99.7	&98	&95.9	 &\textbf{97.3} &	86.7	&98.4	&99.8	&98.2	&98.8	&93.5	&93.3	&94.9	&87.8	&98.4	&93.6	&98.4	&99.7	&98.2	&96	&96.5	&99.7	&98.5	&98.1	&96.5	& \textbf{100} &	98.9	&99.4	&92	&98.5	&93.3	&96.5	&96.7 \\
			UniAD+GAN &99.5	&98.2	&94.6	&96.7	&79.4	&97	&99.2	&98.1	&99	&94	&73.8	&90.3	&86	&97.4	&89.7	&98.3	 &\textbf{99.9} 	&98.1	&91.3	&95.2	&99.9	&98.5	&98.7	&94.7	 &\textbf{100} 	&99	&97.9	&90.1	&97.7	&93.4	&93.8	&95.9 \\
			UniAD+UNet & 99.8	&98.1	&94.6	 &\textbf{97.3} &	86.7	&98.5	&99.9	&98	&99.3	&93.2	&94.8	&95.2	&86.8	&98.3	&94.7	&98.4	&99.8	& \textbf{98.4} 	&95	&96.4	&99.8	&98.5	&97.5	&96.4	 &\textbf{100} 	&98.8	&99.2	&91.9	&98.4	&93.3	&96.4	&96.7 \\
			\midrule
			Ours &  \textbf{100} 	&\textbf{98.5} &	94.7	& {97.2} 	& \textbf{94.0} 	&\textbf{99.0} 	& \textbf{100} 	 &\textbf{98.8} &	 \textbf{99.9} 	 &\textbf{97.5} 	& \textbf{96.9} 	 &\textbf{98.3} &	 \textbf{95.6} 	 &\textbf{99.5} &	 \textbf{100} 	 &\textbf{98.9} 	&99.8	&97.6	 &\textbf{99.7} 	 &\textbf{98.9} 	 &{98.5} 	 &\textbf{98.7} 	&  {99.6} 	& \textbf{98.7} 	& \textbf{100} 	& \textbf{99.2} &	 \textbf{99.9} &	95	& {98.7} &	95.8	 &\textbf{98.5}	& \textbf{98.1}  \\ 
			\bottomrule
	\end{tabular}}
 	\label{tab:mvtec_det}

\end{table*}
